Study of Radiative Decays of Psi(2S) Mesons

We studied the decay psi(2S) to gamma eta_c(2S) with 25.9 million psi(2S) events collected with the CLEO-c detector. No psi(2S) to gamma eta_c(2S) decays were observed in any of the eleven exclusive eta_c(2S) decay modes studied. The product branching fraction upper limits were determined for all modes. The 90% confidence level upper limit of branching fraction of psi(2S) to gamma eta_c (2S) was obtained.

==> signature.tex <==
\begin{center}
  \vfill
  UNIVERSITY OF MINNESOTA
  \vfill
  This is to certify that I have examined this
  copy of a doctoral thesis by \\
  \vfill
  Kaiyan Gao\\
  \vfill
  and have found that it is complete and satisfactory in
  all respects and that any and all revisions required
  by the final examining committee have been made.
  \vfill
  \begin{center}\rule[-5ex]{3.5in}{0.1ex}\end{center}
  Ronald A. Poling\\
  (Faculty Adviser)
  \vfill
  GRADUATE SCHOOL
  \vfill
  % replace with line since we don't know which date he'll sign
  %               \@date
  \begin{center}\rule[-5ex]{2.0in}{0.1ex}\end{center}
  Date
  \vfill
\end{center}
\vfill
\thispagestyle{empty}
\clearpage

